On the interplay between pricing, competition and QoS in ride-hailing

We analyse a non-cooperative game between two competing ride-hailing platforms, each of which is modeled as a two-sided queueing system, where drivers (with a limited level of patience) are assumed to arrive according to a Poisson process at a fixed rate, while the arrival process of (price-sensitive) passengers is split across the two platforms based on Quality of Service (QoS) considerations. As a benchmark, we also consider a monopolistic scenario, where each platform gets half the market share irrespective of its pricing strategy. The key novelty of our formulation is that the total market share is fixed across the platforms. The game thus captures the competition between the platforms over market share, with pricing being the lever used by each platform to influence its share of the market. The market share split is modeled via two different QoS metrics: (i) probability that an arriving passenger obtains a ride, and (ii) the average passenger pick-up time. The platform aims to maximize the rate of revenue generated from matching drivers and passengers. In each of the above settings, we analyse the equilibria associated with the game in certain limiting regimes. We also show that these equilibria remain relevant in the more practically meaningful 'pre-limit.' Interestingly, we show that for a certain range of system parameters, no pure Nash equilibrium exists. Instead, we demonstrate a novel solution concept called an \textit{equilibrium cycle}, which has interesting dynamic connotations. Our results highlight the interplay between competition, passenger-side price sensitivity, and passenger/driver arrival rates.

==> D_metric_WE.tex <==
\section{Duopoly driven by driver unavailability}
\label{sec:pi0}

In this section, we analyse the competition between platforms, using driver unavailability as the QoS metric that governs the Wardrop split of the passenger arrival rate across platforms. Formally, in the language of Section~\ref{sec:model}, this corresponds to~$Q_i = \DA_i$ given in~\eqref{eqn_pi0_expression} for all~$i$. This defines a non-cooperative game between the platforms, wherein platforms use pricing as a lever to influence their market share (and payoffs). The goal of this section is to analyse and interpret the equilibria associated with this game. Our main insight is that when passengers are price-sensitive and scarce (relative to drivers), platforms are forced to deviate from monopoly pricing in order to `fight' for market share, resulting in an equilibrium where both platforms are worse off (relative to the monopolistic scenario).

%The objective of this section is to study the competition between the platforms, as introduced in Section~\ref{sec:model}. Specifically, we focus on addressing passengers' primary concern, which is the unavailability of drivers. To quantify this concern, we define the Quality of Service (QoS) metric (denoted as~$Q_i$) representing the probabilities of driver unavailability~$\{\DA_i\}$. Observe that for any pricing policy~$\VPhi,$ the revenue rate of platform~$i$ (denoted as~$\MR_i(\VPhi; \beta) = \MR_i(\VPhi; \lami, \beta)$) depends upon the passenger arrival rate to the platform, which in turn depends on the Wardrop split. This split, based on the Wardrop Equilibrium (WE), leads to each platform functioning as a separate BCMP network, with the passenger arrival rate determined by the WE.


%We use the blocking probability~$\{\DA_i\}$ to establish the Wardrop split~\eqref{eqn_existence_uniq_WE_main} of the passenger arrival rate across the two platforms. 
%This division leads to a non-cooperative game between the two platforms, thus our goal is to identify the equilibria of this game.
%Nash equilibria of this game in the \idp\ regime and demonstrate that it also qualifies as an~$\epsilon$-NE for sufficiently small~$\beta > 0$.
We begin by characterizing the unique Wardrop Equilibrium (WE) corresponding to any price (action) vector~$\VPhi = (\phi_1, \phi_2)$ in the following lemma (proof in Appendix~\ref{sec:appendix_A}). 

\begin{lemma} \label{lem_pio_WE}
For any~$\beta > 0$ and price vector~$\VPhi \in [0, \phi_h]^2$, the WE under QoS metric~$\DA$ is given by,
\begin{equation*}
  (\lamo, \lamt)   = 
 \left(\frac{\Lambda f(\phi_2)}{f(\phi_1) + f(\phi_2)}, \frac{\Lambda f(\phi_1)}{f(\phi_1) + f(\phi_2)} \right).
\end{equation*}
%Importantly, the WE is insensitive to~$\beta$.   
\end{lemma}
%The above lemma establishes a unique Wardrop Equilibrium (WE) for any given price-vector or strategy profile~$\VPhi$, and~$\beta > 0$. 
Importantly, note that Lemma~\ref{lem_pio_WE} implies that the WE is insensitive to the value of~$\beta$. This allows us to define the WE in the \idp\ regime ($\beta = 0$) as $$\lambda_i(\VPhi; 0) = \frac{\Lambda f(\phi_{-i})}{f(\phi_i) + f(\phi_{-i})}.$$
Consequently, the payoff functions corresponding to the \idp\ regime, defined as the pointwise limits of the payoff functions as~$\beta \downarrow 0,$ are given by: 
%It is worth noting that the passenger distribution resulting from the Wardrop split is independent of the value of~$\beta$ under this QoS metric.
%Consequently,  for small values of~$\beta,$  we approximate the revenue rate of platform~$i$
%using Lemma~\ref{lem_approx_MR} and~\eqref{eq_approx_MR} by direct substitution of~$\lami$ obtained from Lemma~\ref{lem_pio_WE} into~$\lambda_i(\VPhi; 0)$ of Lemma~\ref{lem_approx_MR}
\begin{equation} \label{eqn_MR_d_system_beta_zero}
\MR_i(\VPhi ;0) = \mathds{1}_{\{e < h(\VPhi)\}} e \phi_i  + \mathds{1}_{\{e \geq h(\VPhi)\}} h(\VPhi) \phi_{i},  \text{ where } h(\VPhi) = \lambda_i(\VPhi; 0) f(\phi_i). %= \frac{\Lambda f(\phi_i) f(\phi_{-i})}{f(\phi_i) + f(\phi_{-i})}.
\end{equation}
The above expression follows easily from Lemma~\ref{lem_approx_MR}. %by~$\lami$ obtained from Lemma~\ref{lem_pio_WE}.
%Based on the above revenue rates, we have a non-cooperative `limit game' between the platforms, for which 
We now characterize the (symmetric) equilibria corresponding to the \idp\ regime (i.e., the non-cooperative game defined by the payoff functions~\eqref{eqn_MR_d_system_beta_zero}).

\subsection{Equilibria in the \idp\ regime}

The following theorem provides a complete characterization of the symmetric Nash equilibria (NE) in the \idp\ regime (proof in Appendix~\ref{sec:appendix_A}).

\begin{thm}
\label{thm_uniqueness_symm_NE}
Consider the \idp\ regime~$(\beta = 0)$. Define 
\begin{align*}
\du(\phi):= 2f(\phi) + \phi f'(\phi),\ \phi_u := \max \{ \phi \in [0, \phi_h] : \du(\phi) \geq 0\}.
\end{align*}
%If~$\du(\phi_h) \geq 0$, then set~$\phi_u = \phi_h$~$(\phi_h, \phi_h)~$ is the unique symmetric NE. \\
%Else, i.e., if~$\du(\phi_h) < 0,$ there exists a unique zero~$\phi_d$ of~$\du$ in~$(0,\phi_h)$. In this case,
\begin{enumerate}[$(1)$]
    \item If~$\rho \leq f(\phi_u)/2$, then~$\left( f^{-1}\left(2\rho\right), f^{-1}\left(2\rho \right) \right)$ is the unique symmetric NE;
    \item If~$\rho > f(\phi_u)/2$, then~$(\phi_u,\phi_u)$ is the unique symmetric NE.
\end{enumerate}
\end{thm}

Theorem~\ref{thm_uniqueness_symm_NE} provides insights on how competition between platforms influences their pricing.  Importantly, the equilibrium price quoted by each platform is a decreasing (formally, non-increasing) function of the \dpr~$\rho$. This means that \textit{ as the rate of driver arrivals increases} (or equivalently, as the rate at which passengers enter the system decreases), \textit{the competition between platforms for market share intensifies, resulting in a lower equilibrium price.} 

Next, we formally interpret the equilibrium prices established in Theorem~\ref{thm_uniqueness_symm_NE}. It must be emphasized that while there are clear structural similarities between the statements of Theorem~\ref{thm_uniqueness_symm_NE} and Theorem~\ref{thm_monopoly_opt} (which addresses the optimal monopoly pricing), the quantities~$\dm$ and~$\phi_m$ in the former differ from the corresponding quantities~$\du$ and~$\phi_u$ in the latter. Indeed, it is easy to see that $\du(\cdot) > \dm(\cdot),$ and $\phi_u \geq \phi_m.$ 
%the equilibrium pricing discussed in the previous theorem and the monopoly optimum pricing described in the preceding section are similar, there exists a threshold from which these prices differ. Additionally, we have proven in Lemma~\ref{lem_mono_price_less_than_D} that the equilibrium price in the~$\DA$ system is always equal to or higher than the monopoly price. In fact, the proof of Lemma~\ref{lem_mono_price_less_than_D} demonstrates that~$\phi_u > \phi_m$.
\begin{itemize}
    \item As before, we first consider the special case~$\dm(\phi_h) \geq 0;$ this corresponds the scenario where passengers are relatively price-insensitive.  In this case,~$\phi_u = f^{-1}(2\rho) = \phi_h$, indicating as before that the unique NE corresponds to both platforms charging the maximum permissible price, which is also the optimal monopoly price. In other words, inter-platform competition becomes inconsequential when customers are this insensitive to price; each platform can maximize its profit by charging the highest possible price, regardless of the \dpr.
     %
     %This finding suggests that passengers are relatively insensitive to price changes. In such a scenario, the platforms do not need to compete with each other for market share. Instead, they can maximize their profits by charging the highest possible price, regardless of \dpr.
    \item Next, consider the case~$\dm(\phi_h)< 0$ \&~$\rho \leq f(\phi_u)/2;$ this corresponds to the scenario where passengers are relatively price sensitive, and the \dpr\ is small (i.e., drivers are scarce relative to passengers). In this case, it also holds that~$\rho \leq f(\phi_m)/2;$ this means the equilibrium price coincides with the optimal monopoly price, which is equal to~$f^{-1}(2\rho)$. In other words, \textit{when passengers are price-sensitive, but abundant (relative to drivers), inter-platform competition becomes inconsequential and both platforms operate on monopoly pricing.}
    
    \item Finally, consider the case~$\dm(\phi_h)< 0$ \&~$\rho > f(\phi_u)/2;$ this corresponds to the scenario where passengers are relatively price sensitive, and the \dpr\ is large (i.e., passengers are scarce relative to drivers). In this case, the platforms are forced to compete for market share, and the equilibrium pricing deviates from the optimal monopoly pricing. In other words, \textit{when passengers are price sensitive \textit{and} scarce, competition drives each platform to a sub-optimal price.} In particular, as we show in Lemma~\ref{lem_mono_price_less_than_D} (see Section~\ref{sec:comparison}), the equilibrium price in this case is strictly greater than the monopoly price. Intuitively, this is because platforms try to boost the QoS driver availability (and therefore market share) by \textit{raising} prices (even at the expense of losing some passengers).
    %Here, the unique NE is the unique zero of~$\du(\cdot)$ in the interval~$(0,\phi_h),$ denoted as~$\phi_u$. In this case,~$\rho$ is large, indicating that the drivers are in abundance (i.e., the passengers are scares); thus the platforms do compete for market share, and the equilibrium price differs from the monopoly pricing strategy.
    %Since the passengers QoS is the probability of getting a ride, the platforms are leveraging this fact; thus both the platforms charges the price higher than the monopoly price.
\end{itemize}

In Section~\ref{sec:comparison}, we conduct a comprehensive comparison of the equilibrium prices derived from Theorem~\ref{thm_uniqueness_symm_NE} and the optimal monopolistic price as characterized in Section~\ref{sec:model}. This analysis also sheds light on the welfare implications of platform competition in different market conditions.

\subsection{Applicability of \idp\ equilibria in the pre-limit (i.e., for small~$\beta > 0$)}
%Equilibria in the pre-\idp\ regime~$(\beta > 0)$}

We now establish a connection between the NE in the \idp\ regime (Theorem~\ref{thm_uniqueness_symm_NE}) and equilibrium behavior in the system when~$\beta$ is positive and small. Specifically, we show that the NE in the \idp\ regime is an~$\epsilon$-NE in the pre-limit. We recall here the definition of an $\epsilon$-NE (see~\cite[Section 3.13]{myerson}).

\begin{defn}[$\epsilon$-NE] \label{def_epsilon_equilibria}
Consider a strategic form game~$G = \left< \mathcal{N}, (\Phi_i), (\MR_i)\right>$ where~$\mathcal{N}$ is a finite set, the~$\Phi_i$ are nonempty compact metric spaces, and the~$\MR_i : \Phi_i \to \mathbb{R}$ are utility functions. Given~$\epsilon \geq 0,$ a mixed strategy~$\sigma$ is called an~$\epsilon$-NE if for all~$i \in \mathcal{N}$ and~$\phi_i \in \Phi_i$,
$$
\MR_i(\phi_i, \sigma_{-i}) \leq \MR_i(\sigma_i, \sigma_{-i}) + \epsilon.
$$
Note that when~$\epsilon = 0$, an~$\epsilon$-NE is just an NE in the usual sense.
\end{defn}

%Definition~\ref{def_epsilon_equilibria} introduces the concept of~$\epsilon$-equilibrium in a strategic form game~$G$. The game~$G$ is defined by a finite set of players~$\mathcal{N}$, nonempty compact metric spaces~$\Phi_i$ for each player~$i$, and utility functions~$\MR_i$ mapping strategies to real numbers. In~$\epsilon$-equilibrium a strategy~$\sigma$ that satisfies the condition that for any player~$i$ and strategy~$\phi_i$ of player~$i$, the utility of playing~$\phi_i$ against the other players' strategies~$\sigma_{-i}$ is at most~$\epsilon$ better than the utility of playing~$\sigma_i$ against~$\sigma_{-i}$.
The notion of~$\epsilon$-NE relaxes the notion of the NE in that no player stands to make a utility gain exceeding~$\epsilon$ from a unilateral deviation.

%small deviations from the NE utility.

%It also useful in situations where exact NE may be difficult to find, or may not exist but where small deviations from NE may be acceptable.

\ignore{In Theorem~\ref{thm_uniqueness_symm_NE}, we established the existence of a unique symmetric NE (denote it by~$(\phi^*, \phi^*)$) for the \idp\ regime. Here, we demonstrate that this NE is in fact an~$\epsilon$-NE for the system when~$\beta$ is positive and small.
Towards this, we firstly show in Lemma~\ref{lem_MR_joint_cont} that the function~$\MR$ is jointly continuous with respect to~$(\VPhi, \beta)$ on~$[0, \phi_h]^2 \times [0, \infty)$. Since the driver patience time parameter~$\beta$ can be upper bounded by some large constant~$\bar \beta > 0$, the domain for the revenue rate function~$\MR$ of the platform becomes compact. As a result,~$\MR$ is uniformly continuous on the compact domain~$[0, \phi_h]^2 \times [0, \bar \beta].$ This allows us to approximate the revenue rate with small enough~$\beta$ by the revenue rate when~$\beta = 0$ using uniform continuity.
By leveraging this fact, we demonstrate that when~$\beta = 0$, the NE established in Theorem~\ref{thm_uniqueness_symm_NE} is an~$\epsilon$-NE for small enough~$\beta$.}

\begin{thm} \label{Thm_beta_nonzero_Dsystem}
Consider any~$\epsilon > 0$. There exists~${\bar \beta}_\epsilon >0$ such that for~$0 < \beta \leq {\bar \beta}_\epsilon$, the unique symmetric NE~$(\phi^*, \phi^*)~$ of the \idp\ regime (as characterized in Theorem~\ref{thm_uniqueness_symm_NE}) is an~$\epsilon$-NE.
\end{thm}

Theorem~\ref{Thm_beta_nonzero_Dsystem} (proof in Appendix~\ref{sec:appendix_A}) essentially validates Theorem~\ref{thm_uniqueness_symm_NE}, by showing that the equilibria in the \idp\ regime are also meaningful in the pre-limit (i.e., when $\beta$ is small and positive). In other words, under the assumption of fairly patient drivers, our analysis of the \idp\ regime is indicative of equilibrium behavior of the platforms, and the conclusions of Theorem~\ref{thm_uniqueness_symm_NE} are applicable.

%The above theorem shows that the result obtained at $\beta = 0$ (Theorem~\ref{thm_uniqueness_symm_NE}), where drivers never leave the system due to impatience, holds relatively true even when $\beta$ is small and positive. This implies that the equilibrium state remains relatively unaffected by minor perturbations in the value of $\beta,$ that is under the assumption of highly patient drivers.
%The above theorem shows that the NE obtained from Theorem~\ref{thm_uniqueness_symm_NE} (when $\beta = 0,$ i.e., drivers never leave the system by impatience) is relatively unaffected  when $\beta$ is positive and small i.e., under the assumption of highly patient drivers.

%The above theorem investigates the impact of parameter~$\beta$ on NE, showing that the small perturbation in~$\beta$ from~$\beta = 0$ introduced only negligible perturbation to the NE. This finding demonstrates that the equilibrium state remains relatively unaffected by minor perturbations in the value of~$\beta$.

\ignore{\begin{thm} [$\beta > 0$]  Consider any~$\epsilon > 0$. There exists~${\bar \beta}_\epsilon >0$ such that for~$0 < \beta \leq {\bar \beta}_\epsilon$,
\label{Thm_beta_nonzero_Dsystem}
\begin{enumerate}[$(i)$]
    \item  the unique symmetric NE~$(\phi^*(0), \phi^*(0))~$ of the \idp\ regime (as characterized in Theorem~\ref{thm_uniqueness_symm_NE}) is an~$\epsilon$-NE, and
    \item there exists at least one symmetric NE~$(\phi^*(\beta), \phi^*(\beta))~$ within~$\epsilon$ distance from~$(\phi^*(0), \phi^*(0))~$. \eop    
\end{enumerate}

{\color{blue}{\bf Proof:} The proof is constructed using the following major steps: i) write major steps of the proof here as a proof and then refer the appendix}
\extra{ii) Consider any sequence~$\beta_n \to 0$. There exists  
~$(\phi_n^*, \phi_n^*)~$ a sequence of symmetric NE one corresponding to each~$\beta_n$  such that~$\phi^*_n \to \phi^*$, as~$n \to \infty.$ {\bf Requires additional proof (some sort of diagonal arguments) and to be included only if required..}}{}
\end{thm}

{\color{blue}
\begin{proof}
\noindent \textbf{Case~(ii)}~Theorem~\ref{thm_uniqueness_symm_NE} states the existence and uniqueness of the symmetric NEs for the \idp\ regime.
Here we prove the existence of such NEs in the pre-\idp\ regime, i.e., for~$\beta > 0$. Observe that from Lemma~\ref{lem_deri_mr}, the revenue rate expression for the \idp\ regime is not differentiable on the set~$\mathcal{H}$ as the left limit~($e$) is not same as right limit~($\phi_i h'(\VPhi) + h(\VPhi)$) for all~$\phi_i \in \mathcal{H}$. Similar to Theorem~\ref{thm_uniqueness_symm_NE}, here we consider all three different cases.

\noindent \textbf{Case~$(ii.a)$}~If~$2f(\phi_h) + \phi_h f'(\phi_h) \geq 0$

We find the BR of platform~$1$ (wlog) against~$\phi_2= \phi_h$. Consider a compact domain~$\mathcal{U}_{\epsilon}$ for~$(\phi_1,\beta)$, where
\begin{equation}\label{eqn_u_epsilon}
\mathcal{U}_{\epsilon} :=   [0, \phi_h] \times [0, \bar{\beta}] - {B}\left(\mathcal{H}^h, \nicefrac{\epsilon}{2} \right).
\end{equation}
Where,~${B}\left(\mathcal{H}^h, \nicefrac{\epsilon}{2} \right)$ is an open ball around~$\mathcal{H}^h := \{ (\phi_1, 0) : h(\phi_1, \phi_h) = e\}$ of radius~$\nicefrac{\epsilon}{2}$.  
Note that the function~$\MR(\cdot, \cdot, 0)$ is not differentiable on~$\mathcal{H}^h$. Since~$\mathcal{U}_\epsilon$ is a compact set, using Lemma~\ref{lem_partial_der_cont}, we have that~$\Delta: \mathcal{U}_\epsilon \to \mathbb{R}$ is a uniformly continuous mapping for all~$\epsilon > 0$. Define~$\tilde{\Delta}(\phi,\beta) := \Delta(\phi,\phi_h,\beta)$. Now, it is easy to see that~$\tilde \Delta$ is also uniformly continuous on the set~$\mathcal{U}_\epsilon$. Thus, for any~$\eta >0$, there exists a~$\delta_\eta > 0$  such that 
\begin{equation}
\label{eq_un_cts}
\text{ if } (\phi_1,\beta),(\phi_1',\beta') \in \mathcal{U}_\epsilon \text{ and } \left|(\phi_1,\beta)-(\phi_1',\beta') \right|  \le \delta_\eta \text{ then }
  \left| \tilde{\Delta}(\phi_1,\beta) - \tilde{\Delta}(\phi_1',\beta') \right| \le \eta.
\end{equation}
Further, from Lemma~\ref{lem_deri_mr}, the derivative of revenue rate w.r.t.~$\phi_1$ at~$(\phi_2, \beta) = (\phi_h, 0)$ is~$\left(\text{defined only if }(\phi_1, \beta) \notin B \left(\mathcal{H}^h,\frac{\epsilon}{2}\right) \right)$, 

\begin{equation} \label{eqn_mr_der_positive}
\tilde{\Delta} (\phi_1, 0) = \frac{\Lambda f(\phi_h)}{(f(\phi_1) + f(\phi_h))^2} \left( f(\phi_1) (f(\phi_1) - f(\phi_h)) + f(\phi_h) ( 2f(\phi_1) + f'(\phi_1) \phi_1 )
\right) > l_{\delta} > 0 .
\end{equation}
The above expression can be uniformly lower bounded by~$l_{\delta}$, because under the theorem hypothesis~$2f(\phi_h) + f'(\phi_h) \phi_h > 0$ , and~$f(\phi_1) \geq f(\phi_h)$. Now, consider~$(\phi_1',\beta') = (\phi_1,0) \in \mathcal{U}_\epsilon$ and choose~$\eta =\frac{l_\delta}{2}$ in~\eqref{eq_un_cts}. Then,
there exists a~$\delta_\eta^\epsilon > 0$  such that 
\begin{equation} \label{eqn_uniform_at_zero}
\text{ if } (\phi_1,\beta) \in \mathcal{U}_\epsilon \text{ and } \left|(\phi_1,\beta)-(\phi_1,0) \right|  \le \delta_\eta^\epsilon \text{ then }
  \left| \tilde{\Delta}(\phi_1,\beta) - \tilde{\Delta}(\phi_1,0) \right| \le  \nicefrac{l_\delta}{2}.
\end{equation}

Thus from above, 
$$
\left| \tilde{\Delta}(\phi_1, 0) - \tilde{\Delta}(\phi_1, \beta) \right| \leq \frac{l_{\delta}}{2} \ \ \text{ whenever } \beta \leq  \delta_\eta^\epsilon, \text{ i.e.,} 
$$
$$ \tilde{\Delta}(\phi_1,  \beta) \geq \tilde{\Delta}(\phi_1,  0) - \frac{l_{\delta}}{2} \stackrel{\text{(a)}}{>} \frac{l_{\delta}}{2} > 0 \text{ for all } (\phi_1, \beta) \in \mathcal{U}_\epsilon.$$
Note that the inequality (a) follows from~\eqref{eqn_mr_der_positive}.
Next, we are left to show that~$\tilde{\Delta}(\phi_1,\beta) > 0$ for all~$(\phi_1,\beta) \notin \mathcal{U}_\epsilon.$  For any~$\epsilon > 0$, we have~$\tilde{\Delta}(\phi_1,\beta) > 0$ for all~$(\phi_1,\beta) \in \mathcal{U}_\epsilon.$  From the proof of Theorem~\ref{thm_uniqueness_symm_NE},~$\MR_i(\phi, \phi_h; 0) < \MR_i(\phi_h, \phi_h, 0)$ for all~$\phi \in [0, \phi_h)$ whenever~$2f(\phi_h) + \phi_h f'(\phi_h) > 0$. Thus there exists~$\eta > 0$ such that~$\MR_i(\phi, \phi_h; 0) < \MR_i(\phi_h, \phi_h, 0) - \eta$ for~$\phi \notin \mathcal{U}_\epsilon$. Now, for all~$\phi \notin \mathcal{U}_\epsilon$
\begin{alignat*}{1}
 \MR_i(\phi_h, \phi_h; \beta) - \MR_i(\phi, \phi_h, \beta) & = ( \MR_i(\phi_h, \phi_h; \beta) - \MR_i(\phi_h, \phi_h, 0)) 
 -
 (\MR_i(\phi, \phi_h; \beta) - \MR_i(\phi, \phi_h, 0)) \\
 &\hspace{4.85cm} +
 (\MR_i(\phi_h, \phi_h; 0) - \MR_i(\phi, \phi_h, 0)) \\
& \geq -\eta - (-\eta) + \eta = \eta . 
\end{alignat*}
Using the continuity of~$\MR_i(\phi_1, \phi_h, \beta)$, we can find~$\eta >0$ such that~$\mathcal{M}(\phi_1, \phi_h,\beta)<\mathcal{M}(\phi_h, \phi_h,\beta)-\eta$ for all~$(\phi_1,\beta) \notin \mathcal{U}_\epsilon.$

Thus, the BR of player~$1$ against~$\phi_h$ is~$\phi_h$ and hence,~$(\phi_h, \phi_h)$ is the NE which proves the hypothesis.


\vspace{.3cm}
\noindent\textbf{Case~ii): }
If~$2f(\phi_h) + \phi_h f'(\phi_h) < 0$ and~$\rho \leq f(\phi_d)/2.$

Let~$\tilde \Delta (\phi, \beta) := \Delta (\phi, \phi, \beta)$, and~$\phi^*(\beta)~$ be the zero of~$\tilde \Delta (\phi, \beta)$ if it exists. Consider a compact domain~$\mathcal{U}_{\epsilon}$ for~$(\phi_1,\beta)$, 
\begin{equation}\label{eqn_u_epsilon_two}
\mathcal{U}_{\epsilon} =   [0, \phi_h] \times [0, \bar{\beta}] - {B}\left(\mathcal{H}, \nicefrac{\epsilon}{2} \right) \text{ where } \mathcal{H} := \{ (\phi_1, 0) : h(\phi_1, f^{-1}(2\rho) = e\} \text{ of radius }\nicefrac{\epsilon}{2}.  
\end{equation}
 Similar to previous case, the function~$\tilde \Delta (\phi,  \beta)$ is uniformly continuous over~$\mathcal{U}_{\epsilon}.$
Now to find the symmetric NE, consider
\begin{equation}\label{eqn_par_der_at_phiunderbar}
\tilde \Delta (\phi; 0) = \mathds{1}_{\{e < h(\VPhi)\}} e + \mathds{1}_{\{ e > h(\VPhi)\}} (\Lambda/4)\du(\phi) = \mathds{1}_{\{\phi <   \}} e + \mathds{1}_{\{ \phi >  f^{-1}\left(2\rho\right)\}} (\Lambda/4)\du(\phi).
\end{equation}
$\tilde \Delta (\phi; 0) = e > 0$ for~$\phi <  f^{-1}\left(2\rho\right)$ and as d is decreasing,~$\tilde \Delta (\phi; 0) < 0$ for~$\phi >  f^{-1}\left(2\rho\right)$. Recall that~$\tilde \Delta ( f^{-1}\left(2\rho\right); 0)$ is not defined but~$\MR$ is continuous at~$\phi =  f^{-1}\left(2\rho\right)$. Thus,~$( \phi^*(0),  \phi^*(0))$ is unique symmetric NE for the \idp\ regime. Therefore using ~\eqref{eqn_par_der_at_phiunderbar},~$\tilde \Delta ( \phi^*(0) - \epsilon; 0) > 0$ and~$\tilde \Delta ( \phi^*(0) + \epsilon; 0) < 0$. From Lemma~\ref{lem_partial_der_cont},~$\Delta$ is uniformly continuous over the compact domain~$\mathcal{U}_\epsilon$ and thus~$\tilde \Delta$ is also uniformly continuous. Therefore using uniform continuity of~$\tilde \Delta$, there exists~$\bar \beta_\epsilon$  such that for all~$\beta \leq \bar \beta_\epsilon$, we have~$\tilde \Delta ( \phi^*(0) - \epsilon; \beta) > 0$ and~$\tilde \Delta ( \phi^*(0) + \epsilon; \beta) < 0$. Thus there exist~$ \phi^*(\beta) \in ( \phi^*(0) - \epsilon,  \phi^*(0) + \epsilon)$ such that~$\Delta ( \phi^*(\beta); \beta) = 0$. As~$\du$ is strictly decreasing, the second order conditions are satisfied. Therefore~$( \phi^*(\beta),  \phi^*(\beta))$ is NE.

\vspace{.3cm}
\noindent \textbf{Case~(iii)}
Define~$\tilde \Delta (\phi, \beta) := \Delta (\phi, \phi, \beta)$. Now, for the symmetric NE, it is sufficient to find the zero of~$\tilde \Delta (\phi, \beta)$ ensuring the second order conditions. Consider
\begin{equation}\label{eqn_par_der_at_phido}
\tilde \Delta (\phi; 0) = \mathds{1}_{\{e < h(\VPhi)\}} e + \mathds{1}_{\{ e > h(\VPhi)\}} (\Lambda/4)\du(\phi)
\end{equation}
Recall that~$\du(\phi_d(0)) = 0$ thus,~$(\phi_d(0), \phi_d(0))~$ is an unique symmetric NE for the \idp\ regime. Note that~$\tilde \Delta (\phi; 0) =  (\Lambda/4)\du(\phi)$ at~$\phi = \phi_d(0)$. As~$\du$ is strictly decreasing function, and~$e > h((\phi_d(0), \phi_d(0)))$, there exists~$\epsilon > 0$ such that~$d(\phi_d(0) - \epsilon) > 0$,~$d(\phi_d(0) + \epsilon) < 0$, and still~$e > h((\phi_d(0) - \epsilon, \phi_d(0) - \epsilon))$,~$e > h(\phi_d(0) + \epsilon, \phi_d(0) + \epsilon)$. Therefore using~\eqref{eqn_par_der_at_phido},~$\tilde \Delta (\phi_d(0) - \epsilon; 0) > 0$ and~$\tilde \Delta (\phi_d(0) + \epsilon; 0) < 0$. From Lemma~\ref{lem_partial_der_cont},~$\Delta$ is uniformly continuous over the compact domain~$\mathcal{U}_\epsilon$ and thus~$\tilde \Delta$ is also uniformly continuous. Therefore using uniform continuity of~$\tilde \Delta$, there exists~$\bar \beta_\epsilon$  such that for all~$\beta \leq \bar \beta_\epsilon$, we have~$\tilde \Delta (\phi_d(0) - \epsilon; \beta) > 0$ and~$\tilde \Delta (\phi_d(0) + \epsilon; \beta) < 0$. Thus there exist~$\phi_d(\beta) \in (\phi_d(0) - \epsilon, \phi_d(0) + \epsilon)$ such that~$\Delta (\phi_d(\beta); \beta) = 0$. As~$\du$ is strictly decreasing, the second order conditions are satisfied. Therefore~$(\phi_d(\beta), \phi_d(\beta))$ is NE.



\ignore{
Choose~$\epsilon>0$ such that~$\mathcal{H} \cap \left[ \phido(0)-\epsilon,\phido(0)+\epsilon\right]\times \{\phido(0)\} \times \{0\} = \emptyset$, and this is possible as
$$
\phiunderbar(0) < \phido(0) \implies f(\phido(0)) < \frac{2e}{\Lambda} \implies e > \Lambda f(\phido(0)) - e \implies \frac{e f(\phido(0))}{\Lambda f(\phido(0)) - e} > f(\phido(0)).
$$
Here in the set~$\mathcal{H}$ we have~$\hat \phi$ satisfying~$e = h(\hat \phi, \phido(0))$ which says that~$f(\hat \phi) = \frac{e f(\phido(0))}{\Lambda f(\phido(0)) - e}$. Therefore we have~$f(\hat \phi) > f(\phido(0))$ which means~$\hat \phi < \phido(0)$. Therefore there exists an~$\epsilon > 0$ such that such that~$\mathcal{H} \cap \left[ \phido(0)-\epsilon,\phido(0)+\epsilon\right]\times \{\phido(0)\} \times \{0\} = \emptyset$.}
\end{proof}
}
}


==> references.tex <==
\bibliographystyle{elsarticle-num}
\bibliography{reference.bib}
\ignore{
\begin{thebibliography}{}
\bibitem{TR} Walunj, T.S., Singhal, S., Kavitha, V. and Nair, J., 2022, September. Pricing, competition and market segmentation in ride hailing. In 2022 58th Annual Allerton Conference on Communication, Control, and Computing (Allerton) (pp. 1-8). IEEE.
\bibitem{BCMP_routing} Braverman, A., Dai, J.G., Liu, X. and Ying, L., 2019. Empty-car routing in ridesharing systems. Operations Research, 67(5), pp.1437-1452.
\bibitem{WE_app} Honnappa, H. and Jain, R., 2015. Strategic arrivals into queueing networks: The network concert queueing game. Operations research, 63(1), pp.247-259.
\bibitem{market_share} Singhal, S., Kavitha, V. and Nair, J., 2021, December. Coalition formation in constant sum queueing games. In 2021 60th IEEE Conference on Decision and Control (CDC) (3812-3817). IEEE.
\bibitem{routing} Afimeimounga, H., Solomon, W. and Ziedins, I., 2010. User equilibria for a parallel queueing system with state dependent routing. Queueing Systems, 66(2), pp.169-193.
\bibitem{WE} Correa, J.R. and Stier-Moses, N.E., 2011. Wardrop equilibria. Encyclopedia of Operations Research and Management Science. Wiley.
\bibitem{siva} Varma, S.M., Bumpensanti, P., Maguluri, S.T. and Wang, H., 2022. Dynamic pricing and matching for two-sided queues. Operations Research.
\bibitem{johari} Banerjee, S., Riquelme, C. and Johari, R., 2015. Pricing in ride-share platforms: A queueing-theoretic approach. Available at SSRN 2568258.
\bibitem{uber} Yan, C., Zhu, H., Korolko, N. and Woodard, D., 2020. Dynamic pricing and matching in ride‐hailing platforms. Naval Research Logistics (NRL), 67(8), pp.705-724.
\bibitem{abandon} Nguyen, L.M. and Stolyar, A.L., 2018. A queueing system with on-demand servers: local stability of fluid limits. Queueing Systems, 89(3), pp.243-268.
\bibitem{kaplan} Caldentey, R., Kaplan, E.H. and Weiss, G., 2009. FCFS infinite bipartite matching of servers and customers. Advances in Applied Probability, 41(3), pp.695-730.
%%%%%%%%%%
\bibitem{adan} Adan, I. and Weiss, G., 2012. Exact FCFS matching rates for two infinite multitype sequences. Operations research, 60(2), pp.475-489.
\bibitem{ward} Gurvich, I. and Ward, A., 2015. On the dynamic control of matching queues. Stochastic Systems, 4(2), pp.479-523.
%%%%%%%%%%%%%%%%%%%
\bibitem{pasta} Wolff, R.W., 1982. Poisson arrivals see time averages. Operations research, 30(2), pp.223-231.
\bibitem{BCMP} Baskett, F., Chandy, K.M., Muntz, R.R. and Palacios, F.G., 1975. Open, closed, and mixed networks of queues with different classes of customers. Journal of the ACM (JACM), 22(2), pp.248-260.
\bibitem{protter} Jacod, J. and Protter, P., 2004. Probability essentials. Springer Science \& Business Media.
\bibitem{maximum} Sundaram, R.K., 1996. A first course in optimization theory. Cambridge university press.
\bibitem{balter} Harchol-Balter, M., 2013. Performance modeling and design of computer systems: queueing theory in action. Cambridge University Press.
\bibitem{norris} Norris, J.R. and Norris, J.R., 1998. Markov chains (No. 2). Cambridge university press.
\bibitem{narahari} Narahari, Y., 2014. Game theory and mechanism design (Vol. 4). World Scientific.
%\bibitem{meyn} Meyn, S.P. and Tweedie, R.L., 2012. Markov chains and stochastic stability. Springer Science \& Business Media.
%\bibitem{BCMP} Forest Baskett, K. Mani Chandy, Richard R. Muntz, and Fernando G. Palacios. 1975. Open, Closed, and Mixed Networks of Queues with Different Classes of Customers. J. ACM 22, 2 (April 1975), 248–260. https://doi.org/10.1145/321879.321887.
\bibitem{myerson} Myerson, Roger B., 2007. Game Theory: Analysis of Conflict. Harvard Univ. Press.
\bibitem{rudin} Rudin, W., 1976. Principles of mathematical analysis (Vol. 3). New York: McGraw-hill.
\end{thebibliography}
} %ignore end

==> removed.tex <==
\textbf{Proof of lemma $\ref{lem_mr_derivation}$:} Each platform aims to maximize the individual revenue by matching the driver-passenger pair. The fraction of time spent by the driver in the state $s_i$ over the time $T$ can be given by,
$\frac{\int_0^T \mathbbm{1}_{\{X_i(x_i) = s_i\}}ds}{T}$, where $X_i(x_i)$ denotes state of process at time $x_i$. Consider a renewal cycle where renewal points are denoted by instants when the process returns to state $s_i$. Let the length of the renewal cycle be $\tau_{s_i}$. The reward in a cycle (denoted by $R_{s_i}$) is given by the time spent in state $s_i$ during this cycle. This reward is the exit time from state $s_i$. Suppose this exit time is denoted by $\xi_{s_i}$. 


Let $q_{s_i}$ be the total rate at which any transition occurs in the system when the system is in the state $s_i$.
%{\color{blue}Isn't the part where stationary distribution is equated to long-run average coming from PASTA property?}
\begin{align*}
\pi_i(s_i) &=\lim_{T \rightarrow \infty                     }\frac{\int_0^T \mathbbm{1}_{\{X_i(x_i) = s_i\}}ds}{T} \xrightarrow{\text{RRT}} \frac{1}{\E_{s_i}(\tau_{s_i})q_{s_i}}.
\end{align*}


Here, $\E_{s_i}(\tau_{s_i}) = \frac{1}{q_{s_i}\pi_i(s_i)}$,

$R_{s_i} = \int_0^{\xi_{s_i}} 1 \ ds = \xi_{s_i}$ therefore $\E[R_{s_i}] = \E[\xi_{s_i}] = \frac{1}{q_{s_i}}$.


\subsection*{Revenue generated at platform $i$}
Platform receives no revenue when the waiting driver is not available i.e., $\niw=0$. Let the platform offers the price $\phi_i(\niw)$ when the system is in the state $s_i = (\niw, \nir)$. The matching revenue generated in the renewal cycle starting at $s_i$ is: $\phi_i(\niw) \times \Prob(\text{change is due to passenger arrival)}$.


\begin{align*}
\text{reward in cycle} &= \begin{cases} \phi_i(\niw) & \text{if change is by passenger arrival}, \\ 0 & \text{else.}
\end{cases}.
\end{align*}

Let $R_i(T) $ denote the  total revenue at platform $i$ generated in time $T=[0,t]$ due to matching. Thus,
\begin{eqnarray*}
R_i(T) &=&  \sum_{\niw = 1}^{\infty} \sum_{\nir = 0}^{\infty} R_{s_i = \{\niw, \nir\}} \\
&=& \sum_{\niw = 1}^{\infty} \sum_{\nir = 0}^{\infty} \phi(\niw)\times \Prob_{s_i}\left(\text{passenger arrival}\right) \\
& = & \sum_{\niw = 1}^{\infty} \sum_{\nir = 0}^{\infty} \phi(\niw) \frac{\lambda_i(\niw)}{q_{s_i}},
\end{eqnarray*}
Here, $\lambda_i(\niw)$ denotes the passenger arrival rate when the number of waiting drivers are $\niw$ and $R_{s_i}$ is the matching revenue generated by platform $i$ while in state $s_i$. 
Here we assume that if $\{s_i:\niw = 0\}$ then $R_{s_i} = 0$.
The expected matching revenue is:
\begin{align*}
\text{Matching Revenue} & = \lim\limits_{T \rightarrow \infty} \frac{R_i(T)}{T} , \\
&= \lim\limits_{T \rightarrow \infty}  \sum_{s_i}\frac{ R_{s_i}(T)}{T} , \\
&= \sum_{s_i}\lim\limits_{T \rightarrow \infty}\frac{   R_{s_i}(T)}{T}.
\end{align*}
{\color{red} \textbf{Interchange summation and limits?}}
Here, the long-run revenue earned by the platform $i$ in state $s_i$ is given by,
\begin{align*}
\lim\limits_{T \rightarrow \infty} \frac{R_{s_i}(T)}{T} &\xrightarrow{\text{RRT}} \frac{\E[R_{s_i}]}{\E[\tau_x]},\\ &= \frac{\phi_i(\niw) \frac{\lambda_i(\niw)}{q_{s_i}}}{\frac{1}{q_{s_i}\pi_i(s_i)}},\\
\lim\limits_{T \rightarrow \infty} \frac{R_{s_i}(T)}{T} &= \phi_i(\niw)\pi_i(s_i) \lambda_i(\niw)
\end{align*}
Therefore, expected matching profit is calculated by summing the profit for a particular driver over all the states times the probability of being in the state.
\begin{equation*}
\MR_i = \sum_{s_i: \niw \neq 0} \lim\limits_{T \rightarrow \infty} \frac{R_{s_i}(T)}{T} =  \sum_{s_i} \phi_i(\niw)\pi_i(s_i) \lambda_i
\end{equation*} 

If platform $i$ quotes the price $\phi_i(\niw)$ to the arriving passenger then only $\lambda_i(\niw) f(\phi_i(\niw))$ passenger stream will enter the system and $\lambda_i(\niw) (1 - f(\phi_i(\niw)))$ part of the passenger stream will be blocked due to price. Therefore the matching revenue earned by the platform can be given as:

\begin{equation} \label{eqn_MR_expression}
\MR_i =  \sum_{s_i: \niw \neq 0} \phi_i(\niw)\pi_i(s_i) \lambda_i f(\phi_i(\niw))
\end{equation} 












The blocking probability $\pi(0)$ of a passenger is given by,
\begin{align*}
\pi(0) &= \sum_{r = 0}^{\infty} \pi((0, r)) = C e^{\frac{e}{\nu}} \left(\frac{e^0}{0!} \right) =  \frac{1}{\sum_{n=0}^{\infty} \left[\frac{e^{n}}{\prod_{a=1}^{n}(\frac{\Lambda}{2} f(\phi) + a \beta)}\right]} \\
& \approx \begin{cases}
            1 - \frac{2e}{\Lambda f(\phi)} & \text{ if }  \left(\frac{2e}{\Lambda f(\phi)}\right) < 1, \\
            0 & \text{ else.}
        \end{cases}
\end{align*}



Next we show that $g(0) < 0$ and $g(\Lambda) > 0$. Observe that $g(0) = Q_1(0) - Q_2(\Lambda)$. From \eqref{??}, we have
%\textbf{Claim:} At $\lambda_1 = 0$, $g(0) < 0$ and at $\lambda_1 = \Lambda$, $g(\Lambda) > 0$

\vspace{-4mm}

{\small \begin{align*}
g(0) &=   \left[\sum_{n_1=0}^{\infty} \left(\frac{\eiw^{n_1}}{\prod_{a=1}^{n_1}(a \beta_1)}\right)\right]^{-1} -   \left[\sum_{n_2=0}^{\infty} \left(\frac{\eiw^{n_2}}{\prod_{a=1}^{n_2}(\Lambda f(\phi_i) + a \beta_2)}\right)\right]^{-1}.
\end{align*}}

It suffices to prove the following inequality, 
$$\sum_{n_2=0}^{\infty} \left[\frac{(\eiw)^{n_2}}{\prod_{a=1}^{n_2}(\Lambda f(\phi_i) + a \beta_2)}\right] - \sum_{n_1=0}^{\infty} \left[\frac{\eiw^{n_1}}{\prod_{a=1}^{n_1}(a \beta_1)}\right] < 0.$$ to show that $g(0) < 0$. Simplifying the term on the LHS of the above inequality, we obtain %Note that for any $\beta_i \in [0, \bar{\beta}]$, both of the series are convergent. 
%
\begin{align*}
%&\sum_{n_2=0}^{\infty} \left[\frac{(\eiw)^{n_2}}{\prod_{a=1}^{n_2}(\Lambda f(\phi_i) + a \beta_2)}\right] - \sum_{n_1=0}^{\infty} \left[\frac{(\eiw)^{n_1}}{\prod_{a=1}^{n_1}(a \beta_1)}\right] = \\
& = \sum_{n=0}^{\infty} \left[\frac{\eiw^{n}}{\prod_{a=1}^{n}(\Lambda f(\phi_i) + a \beta_2)} - \frac{\eiw^{n}}{\prod_{a=1}^{n}(a \beta_1)}\right]. \\
& = \sum_{n=0}^{\infty} \eiw^{n} \left[\frac{n!\beta_1^n - \prod_{a=1}^{n}(\Lambda f(\phi_i) + a \beta_2) }{\left(\prod_{a=1}^{n}(\Lambda f(\phi_i) + a \beta_2)\right)\left(\prod_{a=1}^{n}(a \beta_1)\right)} \right].
\end{align*}
For a given pair of $\beta_1, \beta_2$, w.l.o.g., assume that $\beta_1 \leq \beta_2$. Therefore we get
$n!\beta_1^n - \prod_{a=1}^{n}(\Lambda f(\phi_i) + a \beta_2) < 0$. If $\beta_1 > \beta_2$ then defining the function $g(\lambda_2) = Q_1(\Lambda - \lambda_2) - Q_2(\lambda_2)$ and following the above procedure, we will get $g(0) < 0$.
On similar lines, we get $g(\Lambda) = Q_1(\Lambda) - Q_2(0)$ and using similar arguments as above we get $g(\Lambda) > 0$. 

Thus, $g$ satisfies the hypothesis of Intermediate Value Theorem (IVT). Using IVT, there exists a $\lambda_1 = \lambda^* \in (0, \Lambda)$ such that $g(\lambda^*) = 0$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Proof of Lemma \ref{lem_pio_WE}}: %At Wardrop Equilibrium when using $\pi_i(0)$ as a WE metric, the blocking probability of the both the platforms must be same i.e., $\pi_1(0) = \pi_2(0)$. 
From Lemma \ref{lem_exist_unique_WE} we know that there exist an unique WE with $\DA_i$ as a WE metric. Our aim is to find the passenger arrival rate split  at WE $(\lambda_1, \lambda_2)$. 
 
The proof follows by contradiction. If possible, assume $\lambda_1 f(\phi_1) > \lambda_2 f(\phi_2)$  and observe $\lambda_i f(\phi_i)$ is the effective passenger arrival rate to the platform $i \in \mathcal{N}$. Here note that $\lambda_2 = \Lambda - \lambda_1$. Then from Lemma \ref{lem_Montone_with_Arrival_rate}   $N_1 \stackrel{d}{\le} N_2$, i.e., $P (N_1 \ge n) \ge  P (N_2 \ge n)$ for all $n$, where both are the two stationary probabilities. In particular $P(N_1 > 0) \ge P(N_2 > 0)$ and hence   $  \DA_1 = P(N_1=0) <  P(N_2=0) =  \DA_2$.  Thus $(\DA_2-\DA_1) > 0.$
By Lemma \ref{lem_exist_unique_WE}  $\DA_i$ is strictly monotone in $\lambda_i$. Thus one can increase $\DA_1$ and decrease $\DA_2$ by decreasing $\lambda_1$. In all, $\DA_2 - \DA_1$ is a continuous and strictly decreasing function of $\lambda_1$, which 


, which reduces the gap $(\DA_2-\DA_1)^2$, contradicting the definition of WE. 


, which is a contradiction to the definition of WE, which requires $\DA_1 = \DA_2$. 
One can give similar arguments for the case when $\lambda_1 f(\phi_1) < \lambda_2 f(\phi_2)$. 

Thus at WE, the split must be such that $\lambda_1 f(\phi_1) = \lambda_2 f(\phi_2)$. Simplifying it further (using $\lambda_2 = \Lambda - \lambda_1$), we obtain the following: \begin{eqnarray}
%\lambda_1 f(\phi_1) &=& (\Lambda - \lambda_1) f(\phi_2), \nonumber \\
\lamo = \frac{\Lambda f(\phi_2)}{f(\phi_1) + f(\phi_2)} \text{ and } \lamt = \frac{\Lambda f(\phi_1)}{f(\phi_1) + f(\phi_2)}. \nonumber \hspace{10mm}
\text{\eop}
\end{eqnarray}  






\section{Analysis for $f(\phi) = 1 - \frac{\phi}{\phi_h + \epsilon}$}
\begin{enumerate}
\item $\phimr := {\arg \max}_{\phi \in [0, \phi_h]} \{\Lambda f(\phi) \phi - e\phi\}$
    
$m(\phi) = \Lambda f(\phi) \phi - e\phi.$ By differentiating the function $m$, we get $m'(\phi) = \Lambda - e -  \Lambda \frac{2 \phi}{\phi_h + \epsilon}$. By equating $m'(\phi) = 0$, we get $ \phimr = \frac{\Lambda - e}{2\Lambda}(\phi_h + \epsilon) = \left(\frac{1 - x}{2} (\phi_h + \epsilon) \right)$.  Since $m''( \phimr) < 0$, $\phimr$ is maximizer of the function $m$.
    
    
\item $\phifp := {\arg \max}_{\phi \in [0, \phi_h]} \{f(\phi) \phi\}$
    
Let $\P(\phi) = f(\phi) \phi$. By differentiating the function $\P$, we get $\P'(\phi) = 1 - \frac{{2\phi}}{\phi_h + \epsilon}$. By equating $\P'(\phi) = 0$, we get $\phifp = \frac{\phi_h + \epsilon}{2}$. Since $\P'(\phifp) < 0$, $\phifp$ is maximizer of the function $\P$.

    
\item $\phibar = f^{-1}\left( \frac{e}{\Lambda}\right) \implies f(\phibar) =  \frac{e}{\Lambda} \implies 1 - \frac{\phibar}{\phi_h + \epsilon} =  \frac{e}{\Lambda} \\ \therefore \phibar = \left( 1 - \frac{e}{\Lambda}\right)(\phi_h + \epsilon) $.
    
    
\item $\phiunderbar = f^{-1}\left( \frac{2e}{\Lambda}\right)\implies f(\phiunderbar) =  \frac{2e}{\Lambda} \implies 1 - \frac{\phiunderbar}{\phi_h + \epsilon} =  \frac{2e}{\Lambda} \\ \therefore \phiunderbar = \left( 1 - \frac{2e}{\Lambda}\right)(\phi_h + \epsilon) $. (possible only if $\Lambda > 3e$)

\item $\eL = \frac{\mstar}{e} = \frac{m(\eU)}{e} = \frac{(\Lambda - e)^2}{4e\Lambda}(\phi_h + \epsilon) = \frac{(\phi_h + \epsilon)}{4}\left( \frac{1}{x} -2 + x\right)$.
\item $\phido = \frac{2 (\phi_h + \epsilon)}{3}$ 

$d(\phido) = 2 - \frac{3\phido}{\phi_h}$
\end{enumerate}



\section{Analysis for $f(\phi) = 1 - \sqrt{\frac{\phi}{\phi_h + \epsilon}}$}
\begin{enumerate}
    \item $\phimr := {\arg \max}_{\phi \in [0, \phi_h]} \{\Lambda f(\phi) \phi - e\phi\}$
    
    Let $g_1(\phi) = \Lambda f(\phi) \phi - e\phi.$ Therefore $g_1(\phimr) = \Lambda \phimr - \Lambda \phimr \sqrt{\frac{\phimr}{\phi_h + \epsilon}} - e\phimr$. Taking derivative of the function $g_1$ and equating it to zero, we get $g_1'(\phimr) = \Lambda - e -  \frac{3\Lambda}{2} \sqrt{\frac{ \phimr}{\phi_h + \epsilon}} = 0$
    
    $\therefore \phimr = \left(\frac{2(\Lambda - e)}{3\Lambda}\right)^2(\phi_h + \epsilon) = \frac{4}{9}(1 - x)^2 (\phi_h + \epsilon)$
    
    
    \item $\phifp := {\arg \max}_{\phi \in [0, \phi_h]} \{\Lambda f(\phi) \phi\}$
    
    Let $g_2(\phi) = \Lambda f(\phi) \phi.$ Therefore $g_2(\phifp) = \Lambda \phifp - \Lambda \phifp \sqrt{\frac{\phifp}{\phi_h + \epsilon}}$. Taking derivative of the function $g_2$ and equating it to zero, we get $g_2'(\phifp) = \Lambda -   \frac{3\Lambda}{2} \sqrt{\frac{ \phifp}{\phi_h + \epsilon}} = 0$
    
    $\therefore \phifp = \frac{4}{9}(\phi_h + \epsilon)$
    
    
    \item $\phibar = f^{-1}\left( \frac{e}{\Lambda}\right) \implies f(\phibar) =  \frac{e}{\Lambda} \implies 1 - \sqrt{\frac{\phibar}{\phi_h + \epsilon}} =  \frac{e}{\Lambda} \\ \therefore \phibar = \left( 1 - \frac{e}{\Lambda}\right)^2 (\phi_h + \epsilon) $.
    
    
    \item $\phiunderbar = f^{-1}\left( \frac{2e}{\Lambda}\right)\implies f(\phiunderbar) =  \frac{2e}{\Lambda} \implies 1 - \sqrt{\frac{\phiunderbar}{\phi_h + \epsilon}} =  \frac{2e}{\Lambda} \\ \therefore \phiunderbar = \left( 1 - \frac{2e}{\Lambda}\right)^2 (\phi_h + \epsilon) $.
    
    \item $\eL = \frac{\mstar}{e} = \frac{m(\eU)}{e} = \frac{4(\Lambda - e)^3}{27e\Lambda^2}(\phi_h + \epsilon) = \frac{4}{27} (\phi_h + \epsilon) \left( \frac{1}{x} - x^2 - 3 + 3x\right)  $.
    \item $\phido = \frac{16 (\phi_h + \epsilon)}{25}$
\end{enumerate}


\subsection{Simulation - NE for $\beta \approx 0 \ \ \& \ \ \beta > 0 $ are matching}



\



\ignore{\begin{equation}
\DAl_i = \begin{cases}
    1 - \frac{\eiw}{\lami f(\phi_i)} & \text{ if }  \left(\frac{\eiw}{\lami f(\phi_i)}\right) < 1, \\
           0 & \text{ else.}
   \end{cases} 
\end{equation}}

Limit system ($\bbeta=0$)
W.l.o.g. when $\phi_1>\phi_2$,
\begin{equation}
    WE_1 = \begin{cases}
  \lamo   & \text{ if } \frac{e}{(\lami f(\phi_i))}<1 \text{ for } i= \{1,2\} \\
  \lamo & \text{ if } \frac{e}{\lami f(\phi_i)}\ge 1 \text{ for } i= \{1,2\} 
    \end{cases}
\end{equation}
We proved WE is continuous in $\bbeta$ for all $\bbeta > 0$. Then the following limits exist:
$$
\lambda_i^*(\VPhi) := \lim_{ \bbeta \to (0,0) } \lami  
$$

At WE we have for any $\bbeta > 0$ (only stability is required, which is always true when $\bbeta > 0$ )
$$
\lambda_1 f(\phi_1) = \lambda_2 f(\phi_2)  
$$
Therefore WE split does not depend upon $\bbeta$ and hence easy to define
$$
\lambda_i^*(\VPhi) :=   \lami  
$$

Thus WE of limit system coincides with limit of the WE (when the first condition in (8) is true)



Since the derivative of the function $h$ is continuous, we will only focus on the infinite series. For any $i\in \mathcal{N}, \ \phi_{i,m} \in [0, \phi_h]$ and $ \beta_{m} \in [0, \infty)$, 
$\text{ consider } (\phi_{1,m}, \phi_{2,m}, \beta_m) \rightarrow (\phi_1, \phi_2, \beta).$
We know $\beta_m \to \beta$ and thus, for any $\epsilon > 0$, there exists a $N_\epsilon \in \mathbb{N}$ s.t. for all $m \geq N_\epsilon$, we have $\beta-\epsilon \le \beta_m \le \beta+ \epsilon.$ Therefore, for all $m \geq N_\epsilon$, we have $e/\beta_m\leq e/(\beta-\epsilon)$.

\begin{align*}
\sum_{n=1}^{\infty} \left[
\prod_{a = 1}^n \frac{e}{h(\VPhi_m) + a \beta_m} \left( \sum_{j=1}^n \frac{1}{h(\VPhi_m) + j \beta_m} \right)
\right]
&\leq
\sum_{n=1}^{\infty} \left[
\prod_{a = 1}^n \frac{e}{a \beta_m} \left( \sum_{j=1}^n \frac{1}{ j \beta_m} \right)
\right]
\leq 
\sum_{n=1}^{\infty} \left[
\prod_{a = 1}^n \frac{e}{a (\beta - \epsilon)} \left( \sum_{j=1}^n \frac{1}{ j (\beta - \epsilon)} \right)
\right] \\
&= \left(\frac{e}{(\beta - \epsilon)^2}\right)^2 \sum_{n=1}^{\infty} \left[
 \frac{1}{a!} \left( \sum_{j=1}^n \frac{1}{ j} \right)
\right]
\end{align*}
Note that the series in the right hand side is converging. Therefore, there exists a finite uniform upper bound on the given infinite series sum. Thus using dominated convergence theorem,
\begin{align*}
\sum_{n=1}^{\infty} \left[
\prod_{a = 1}^n \frac{e}{h(\VPhi_m) + a \beta_m} \left( \sum_{j=1}^n \frac{1}{h(\VPhi_m) + j \beta_m} \right)
\right] \longrightarrow
\sum_{n=1}^{\infty} \left[
\prod_{a = 1}^n \frac{e}{h(\VPhi) + a \beta} \left( \sum_{j=1}^n \frac{1}{h(\VPhi) + j \beta} \right)
\right]
\end{align*}
Therefore, $\frac{\partial}{\partial \phi_i} \left( \sum_{n=0}^{\infty} \mu_n \right)$ converges uniformly and $\frac{\partial}{\partial \phi_i} \left( \sum_{n=0}^{\infty} \mu_n \right) = \left( \sum_{n=0}^{\infty} \frac{\partial}{\partial \phi_i}  \mu_n \right)$
}



\ignore{\textbf{Proof of Theorem \ref{thm_B_sys_limit_sys_main}: }
The matching revenue of any platform depends on the obtained passenger arrival rate split through WE, which in turn depends on the prices offered by both platforms. Therefore using Lemmas \ref{lem_approx_MR} and \ref{lem_pio_WE}, the matching revenue of platform $i$ is:
\begin{align}
    \MRl_i(\VPhi) &=   \begin{cases}
        \eiw \phi_i & \text{ if }  e\phi_i < h(\phi_i, \phi_{-i}), \\
        h(\phi_i, \phi_{-i}) & \text{ else.}
    \end{cases} \label{eqn_thm_pio_mr_1} \\
    &= {\min}\left \{e\phi_i, h(\phi_i, \phi_{-i})\right \} \label{eqn_thm_pio_mr_2}
\end{align} 
Here, $h(\phi_i, \phi_{-i}) = \frac{\Lambda f(\phi_i)f(\phi_{-i}) \phi_i}{f(\phi_i) + f(\phi_{-i})}$.
By \textbf{A.1}, the denominator of the function $h$ is never zero and therefore $\MRl_i$ is continuous function of $\phi_i$. To optimize $\MRl_i$, we find the partial derivative of $h$ w.r.t. $\phi_i$.

\vspace{-4mm}

{\small
\begin{align}
 \frac{\partial }{\partial \phi_i}h(\phi_i, \phi_{-i})
&= \Lambda f(\phi_{-i}) \frac{f(\phi_i)^2 + f(\phi_i)f(\phi_{-i}) + \phi_i f'(\phi_i) f(\phi_{-i})}{\left(f(\phi_i) + f(\phi_{-i})\right)^2}. \label{eqn_partial_derivative_MR}
\end{align} }
From  \textbf{A.1}, like $f$,  $f^2$ is also strictly concave and decreasing function; further, by strict concavity of  $f$, derivative $f'$ is negative and decreasing, and therefore $\phi_i \mapsto f'(\phi_i)\phi_i$ is strictly decreasing function. Thus for a given fixed $\phi_{-i}$, the numerator of  partial derivative of   $h$ given in \eqref{eqn_partial_derivative_MR}  
is strictly decreasing  in $\phi_i$. 


Case (i) Fix $\phi_{-i} = \phiunderbar$. If $\frac{\partial }{\partial \phi_i}h(\phiunderbar, \phiunderbar) \leq 0$ then using the monotonicity of the numerator of the derivative in \eqref{eqn_partial_derivative_MR}, the numerator
$$
f(\phi_i)^2 + f(\phi_{-i}) \bigg ( f(\phi_i) + \phi_i f'(\phi_i) \bigg) < 0 \mbox{ for all } \phi_i > \phi_{-i}
$$
 with $\phi_{-i} = \phiunderbar$, then the function $h$ is decreasing after $\phiunderbar$. Therefore $(\phiunderbar, \phiunderbar)$ is a NE if 
 $$
 f(\phiunderbar)^2 + f(\phiunderbar) \bigg ( f(\phiunderbar) + \phiunderbar f'(\phiunderbar) \bigg) \leq 0 $$ $$\mbox{ or equivalently }
 \frac{4e}{\Lambda} +  \phiunderbar f' ( \phiunderbar) \leq 0.
 $$
 Thus  $d (\phiunderbar) \le  0$ iff $(\phiunderbar, \phiunderbar)$ is NE.



{ \color{blue}We are interested in a symmetric NE, so we find a $\phi$ such that $\phi$ is in the BR against itself, i.e., such that $\phi \in \arg \max_{\phi_i} \MRl_i (\phi_i, \phi_{-i})$ with $\phi_{-i}=\phi$.
Thus, to begin with, we need to find 
zeros of the following constructed using   \eqref{eqn_partial_derivative_MR}:
\begin{align}
\left .
 \frac{\partial }{\partial \phi_i}h(\phi_i, \phi_{-i}) \right |_{(\phi_i, \phi_{-i}) = (\phi, \phi)} = 0 \mbox{ or equivalently }
  \frac{\Lambda}{4} \left( 2 f(\phi) + f'(\phi) \phi \right) = 0.
\end{align}
The solution of any $\phi > \phiunderbar$ leads to NE (if further second order conditions are shown). 
 

{\bf Case when $(\phiunderbar, \phiunderbar)$ is NE}
If numerator of the derivative in \eqref{eqn_partial_derivative_MR}   
$$
f(\phi_i)^2 + f(\phi_{-i}) \bigg ( f(\phi_i) + \phi_i f'(\phi_i) \bigg) < 0 \mbox{ for all } \phi_i \ge \phi_{-i}
$$
 with $\phi_{-i} = \phiunderbar$, then $(\phiunderbar, \phiunderbar)$ is NE. {\color{red}By strict concavity provided by {\bf A}.1, the above is strictly decreasing beyond $\phiunderbar$} and then the function $h$ is decreasing after $\phiunderbar$ if the above expression is negative at $\phiunderbar$.
 
 
 Therefore $(\phiunderbar, \phiunderbar)$ is a NE if 
 $$
 f(\phiunderbar)^2 + f(\phiunderbar) \bigg ( f(\phiunderbar) + \phiunderbar f'(\phiunderbar) \bigg) \leq 0 $$ $$\mbox{ or equivalently }
 \frac{4e}{\Lambda} +  \phiunderbar f' ( \phiunderbar) \leq 0.
 $$
 Thus  $d (\phiunderbar) \le  0$ iff $(\phiunderbar, \phiunderbar)$ is NE.
 
 Now consider the case when $d(\phiunderbar) >  0$. 
 Before proceeding, observe   that  for any $\phi_i \in [\phiunderbar, \phi_h]$, as $f(\phi_i) < \frac{2e}{\Lambda}$  and hence,
 \begin{align*}
     h(\phi_i, \phi_i) = \frac{\Lambda f(\phi_i)\phi_i}{2} 
     < e \phi_i, \mbox{ so, }
      \MRl (\phi_i, \phi_i) = h(\phi_i, \phi_i) .
 \end{align*}
 Also observe that $\MRl(\phi, \phi_i) < \MRl (\phiunderbar, \phi_i)$ for any $\phi \le \phiunderbar$.
 
 When $d(\phiunderbar) >  0$
 and  $d(\phi_h) < 0$ 
 then intermediate value theorem, there exists a root $\phido$ s.t. $d(\phido) = 0$, as $d$ is continuous by {\bf A}.1. Thus   $\phido$ is maximizer of the function $h (\cdot, \phido)$  and hence that of $\MRl (\cdot, \phido)$ (if second order conditions) ... Thus $(\phido, \phido)$ is NE if $d(\phiunderbar) >  0$
 and  $d(\phi_h) < 0$.
  
 
 }

\newpage 

Let the function $d(\phi) = (2f(\phi) + \phi f'(\phi))$. From Lemma \ref{lem_monotonicity_of_h_1_function}, we know that $d(\phi)$ is monotonically decreasing function. If there exists a point $\phido \in [0, \phi_h]$ s.t. $d(\phi) = 0$ then $\phido$ is the extreme point of function $h$ and using strict concavity, $\phido$ is the maximizer of function $h$.





If $d(\phiunderbar) \leq 0$ then it shows that the derivative of the function $h$ is negative after $\phiunderbar$ i.e., $\phido \leq \phiunderbar$. Therefore using continuity of $\MRl_i$, we get $\phiunderbar$ as the best response of player $i$ against the opponent's strategy $\phi_{-i} = \phiunderbar$. Therefore $(\phiunderbar, \phiunderbar)$ is a NE.

Note that at given any point $\phi_i \in (\phiunderbar, \phi_h]$, $\phi_i > \frac{2e}{\Lambda}$ therefore we have $f(\phi_i) < \frac{2e}{\Lambda}$ i.e., $\frac{\Lambda f(\phi_i)}{2} < e$ or $\frac{\Lambda f(\phi_i)\phi_i}{2} < e\phi_i$ but $h(\phi_i, \phi_i) = \frac{\Lambda f(\phi_i)\phi_i}{2} < e\phi_i$. Thefore for any $\phi_i \in (\phiunderbar, \phi_h], h(\phi_i, \phi_i) < e\phi_i$.


If $d(\phi_h) \ge 0$ then it shows that the derivative of the function $h$ is non-negative throughout. Therefore $\phi_h$ is the best response of player $i$ against the opponent's strategy $\phi_{-i} = \phi_h$. Therefore $(\phi_h, \phi_h)$ is a NE.

If $d(\phiunderbar) > 0$ and $d(\phi_h) < 0$ then  using continuity of the function $d$, using intermediate value theorem, there exits a root $\phido$ s.t. $d(\phido) = 0$. Therefore $\phido$ is maximizer of the function $h$ and $\phiunderbar < \phido$. Using continuity of the function $\MRl$, $\phido$ is the best response of player $i$ against the opponent's strategy $\phi_{-i} = \phido$. Therefore $(\phido, \phido)$ is a NE. 
\eop


{\color{red}
If $\phiunderbar > \max_{\phi\geq \phiunderbar}\{\frac{2f(\phi)\phi}{f(\phi) + \frac{2e}{\Lambda}}\}$ then $(\phiunderbar, \phiunderbar)$ is a NE. 
The derivative of the latter function is given by

$$2e \frac{f(\phi)^2 + f(\phi)\frac{2e}{\Lambda} + \phi f'(\phi) \frac{2e}{\Lambda}}{\left(f(\phi) + \frac{2e}{\Lambda}\right)^2}
$$

In fact 
$
\frac{4e}{\Lambda} + \phiunderbar f' (\phiunderbar) < 0
$
iff $(\phiunderbar, \phiunderbar)$ is a NE


Most probable result is:
 $(\phiunderbar, \phiunderbar)$ is a NE if
$
\frac{4e}{\Lambda} + \phiunderbar f' (\phiunderbar) < 0
$
else $ (\phido, \phido)$ is NE (or $(\phi_h, \phi_h) is NE$ 


}


\begin{eqnarray}
%\lambda_1 f(\phi_1) &=& (\Lambda - \lambda_1) f(\phi_2), \nonumber \\
\lamo = \frac{\Lambda f(\phi_2)}{f(\phi_1) + f(\phi_2)} \text{ and } \lamt = \frac{\Lambda f(\phi_1)}{f(\phi_1) + f(\phi_2)}. \nonumber
\end{eqnarray}

$$
\frac{e(f(\phi_i)+f(\phi_{-i}))}{\Lambda f(\phi_i)f(\phi_{-i})} \quad \phiunderbar = f^{-1}\left( \frac{2e}{\Lambda} \right)
$$

{\color{red}Note that the entry in the second row follows}

\textbf{When ${\eiw} \geq {\lami f(\phi_i)}$:} From \eqref{eqn_mr_expression_pio} and Lemma \ref{lem_pio_WE}, the optimum matching revenue in this case is attained at the price $$\phiistar = \arg \max_{\phi_i}\left(\frac{\Lambda f(\phi_i)f(\phi_{-i}) \phi_i}{f(\phi_i) + f(\phi_{-i})}\right).$$ %where $h(\phi_i) = \lami f(\phi_i) \phi_i = \frac{\Lambda f(\phi_i)f(\phi_{-i}) \phi_i}{f(\phi_i) + f(\phi_{-i})}$ and the term $\lambda_i(\VPhi) = \frac{\Lambda f(\phi_{-i})}{f(\phi_i) + f(\phi_{-i})}$ comes from the lemma \ref{lem_pio_WE}. 
To obtain $\phiistar$, we differentiate the function on RHS of the above equation in the following,
\begin{align*}
 \frac{d}{d\phi_i}\left(\frac{\Lambda f(\phi_i)f(\phi_{-i}) \phi_i}{f(\phi_i) + f(\phi_{-i})}\right) := \\
& \hspace{-38mm}= \Lambda f(\phi_{-i}) \frac{\left[ f(\phi_i) + f(\phi_{-i}) \right] \left[f(\phi_i) + \phi_i f'(\phi_i) \right] -  \left[ f(\phi_i) \phi_i \right]  \left[ f'(\phi_i) \right]}{\left(f(\phi_i) + f(\phi_{-i})\right)^2}. \\
& \hspace{-38mm}= \Lambda f(\phi_{-i}) \frac{f(\phi_i)^2 + f(\phi_i)f(\phi_{-i}) + \phi_i f'(\phi_i) f(\phi_{-i})}{\left(f(\phi_i) + f(\phi_{-i})\right)^2}.
\end{align*}
Since the platforms are assumed to be symmetric, we have $\phi_i = \phi_{-i}$, which implies $f(\phi_i) = f(\phi_{-i})$. By equating the above derivative to zero we obtain,
\begin{eqnarray*}
%2f(\phi_i)^2 + \phi_i f(\phi_i) f'(\phi_i) &= 0 \nonumber \\ 
f(\phi_i) (2f(\phi_i) + \phi_i f'(\phi_i)) = 0.
\end{eqnarray*} 
From assumption \textbf{A.1}, we know that $ f(\phi) \neq 0 \text{ for all } \phi \in [0, \phi_h].$ Hence, we require a $\phi_i$ which satisfies,
\begin{eqnarray}
\label{eqn_derivative_of_WE_lambda}
d(\phi_i) = (2f(\phi_i) + \phi_i f'(\phi_i)) = 0.
\end{eqnarray}
%Here note that  $d(\phi_i) =  (2f(\phi_i) + \phi_i f'(\phi_i))$. 


\textbf{When $e < \lami f(\phi_i)$:} From \eqref{eqn_mr_expression_pio}, the optimum matching revenue in this case is attained at the price
$$
\phiistar = \arg \max_{\phi_i} e\phi_i
$$
%the platform generates the matching revenue $e\phi_i$. 
Since $e\phi_i$ is a linearly increasing function, the maximum of the matching revenue $e\phi_i$ is attained at $\phiunderbar^-$ (see \eqref{eq_pio_proof_mr}). %when $e\phi_i = \lami f(\phi_i) \phi_i$ i.e., $e = \lami f(\phi_i)$. 
{\color{red}Since we use symmetric pricing policies for the platforms, we split the arrival rate $\Lambda$ s.t.
$\lami = \frac{\Lambda}{2}$ i.e., $e =  \frac{\Lambda}{2} f(\phi_i)$ or $\phi_i = \phiunderbar$. Therefore the platform gets the matching revenue $e\phi_i$ for $\phi_i \in [0, \phiunderbar]$.} %The matching revenue of the platforms as given in \eqref{eqn_mr_expression_pio} by playing different  strategies is given below:
%\begin{equation} \label{eq_pio_proof_mr}
%\MR_i(\phi_i) \approx   \begin{cases}
      %  \eiw \phi_i & \text{ if }  \phi_i \in [0, \phiunderbar), \\
     %  \frac{\Lambda}{2}f(\phiunderbar) \phiunderbar = \frac{\Lambda}{2}\frac{2e}{\Lambda} \phiunderbar  = e\phiunderbar & \text{ if }  \phi_i = \phiunderbar, \\
    %    \lami f(\phi_i) \phi_i & \text{ else.}
  %  \end{cases}
%\end{equation}

\textbf{Proof to else part:} If  $d(\phi_h) > 0$. From Lemma \ref{lem_monotonicity_of_h_1_function}, we know that $d(\phi_i)$ is monotonically decreasing function. Since $d(\phi_h) > 0$, which means that $d(\phi_i) > 0$ for all $\phi_i \in [0, \phi_h]$ and hence the derivative of the function $h(\phi_i)$ is positive throughout. Therefore the maximum of the function $\MR_i(\phi_i)$ is at the rightmost point, which is $\phi_h$. Here note that the maximizer of $e\phi_i$ is at $\phiunderbar$ and from equation \eqref{eq_pio_proof_mr}, $\MR_i(\phiunderbar) < \MR_i(\phi_h)$.


\textbf{Proof of part (a) }\textbf{Case 1: When $\phiunderbar < \phido \le \phi_h $}

As given in equation \eqref{eqn_derivative_of_WE_lambda}, there exists a $\phido \in [0, \phi_h]$ s.t. $2f(\phido) + \phido f'(\phido) = 0$. From Lemma \eqref{lem_monotonicity_of_h_1_function}, we know that $d(\phi)$ is monotonic function $\forall \phi \in [0, \phi_h]$. Therefore this $\phido$ is unique maximizer of the function $h(\phi_i)$. Given that $\phiunderbar < \phido$ and the maximizer of $h(\phi)$ is $\phido$, we have $e\phiunderbar = \frac{\Lambda}{2}f(\phiunderbar) \phiunderbar < \frac{\Lambda}{2}f(\phido)\phido$. Therefore in this case the platform will always find beneficial to choose the pricing policy $\phido$ to maximize the revenue. Since both platforms are symmetric, both of them will choose $\phido$ as unilateral deviation is not better since $\phido$ is a maximizer of the function $h(\phi)$. Therefore $(\phido, \phido)$ is a NE.

\textbf{Case 2: When $0 \le \phido \le \phiunderbar$}

As given in part (b), there exist a unique maximizer $\phido$ of the function $h(\phi)$. Given that $\phiunderbar \geq \phido$ and from equation \eqref{eq_pio_proof_mr}, we know that when $\phi_i \in [0, \phiunderbar]$, the matching revenue of the platform is $e\phi_i$. From equation \eqref{eq_pio_proof_mr}, $h(\phiunderbar)  = e\phiunderbar$ and after $\phiunderbar$, the function $h(\phi)$ decreases as $\phido \leq \phiunderbar$ and $h'(\phi)$ is monotone. Therefore in this case the platform will always find beneficial to choose the pricing policy $\phiunderbar$ to maximize the revenue. Since both platforms are symmetric, both of them will choose $\phiunderbar$ as unilateral deviation is not better since $\phiunderbar$ is a maximizer of the function $e \mapsto e\phi$ over $\phi \in [0, \phiunderbar]$. Therefore $(\phiunderbar, \phiunderbar)$ is a NE.

\textbf{Proof of part (b):} As $e > \Lambda$, we have $e > \lami f(\phi_i)$ for all $\phi_i \in [0, \phi_h]$. Therefore the platform gets the matching revenue $h(\phi_i)$ for all $\phi in [0, \phi_h]$. The maximum of the function $h(\phi)i)$ is at point $\phido$ and because of symmetric nature, we have $(\phido, \phido)$ as a NE.}


\ignore{In this case any~$\lamo$ optimizes~\eqref{eqn_existence_uniq_WE_main}. 
Thus, we consider the following as limit WE:  
$$(\lamol, \lamtl) = \left(0, \Lambda \right),$$
and show that the selection ensures the required continuity properties. Towards this, consider any $\beta_n \to 0$ and consider corresponding $\lim_{\beta_n \to 0} \lambda_1(\VPhi; \beta_n)$. We claim that $\lambda_1(\VPhi; \beta_n) \to 0$, which we prove case-wise as below:
%i.e., the platform with the minimum blocking probability obtains the entire arriving streams of passengers. 
%To show the uniqueness of WE in this case, one needs to show that the WE $(\lamo,\lamt)$ corresponding to the sequence of $\beta_n \to 0$  converges to $(0,\Lambda)$, when $\phi_1 \in [\phibar, \phi_h]$ and $\phi_1>\phi_2$.
  
When $\phi_2 \in [f^{-1}\left( \rho \right), \phi_h]$:
Consider any $\epsilon >0.$
By   Lemma \ref{lem_approx_MR}, with $\lambda_i(\beta) = 0$
for all $\beta$,     
  there exists a $\beta_\epsilon$ such that 
  $$\DA_1 (\phi_1; 0, \beta) \le \epsilon/f(\phi_1)  \mbox{ and hence }
  \PB_1(\phi_1; 0,\beta) < 1-f(\phi_1) + \epsilon$$
  for all  $\beta \le \beta_\epsilon$ (see   \eqref{Eq_overall_exact}). In similar lines,  
  $$\PB_2(\phi_2; \Lambda,\beta) > 1-f(\phi_2)-\epsilon, \mbox{ when } \beta \le \beta_\epsilon.$$  This implies $\PB_1(\lambda;\beta) < 1-f(\phi_1) + \epsilon$ and $\PB_2(\lambda;\beta) \ge 1-f(\phi_2)-\epsilon$ respectively, for all $\lambda$. 
  %
For all such $0 < \beta \le \beta_\epsilon$ from \eqref{eqn_existence_uniq_WE_main},
$W(\beta)  = (0, \Lambda)$, if $\epsilon < (f(\phi_2) - f(\phi_1))/4$.

One can give similar arguments for the other case, now with $\PB_2(\phi_2;\Lambda,\beta) \to 1-\nicefrac{e}{\Lambda f(\phi_2)}$.
%\textbf{Case 2: When $f(\phi_2) > \nicefrac{e}{\lambda}$:}
This completes the proof of claim. 
Substituting this WE in Lemma \ref{lem_approx_MR}, the matching revenue is,
$$
(\MR_1(\VPhi; 0),\MR_2(\VPhi; 0)) = (0,\min \{\Lambda f(\phi_2),e\} \phi_2). 
$$

Using the continuity of WE, we prove the joint continuity of $\MR$ with respect to $(\lambda_1, \lambda_2, \beta).$ For any $(\lambda_1, \lambda_2, \beta) \in [0, \phi_h]^2 \times [0, \infty),$ the matching revenue of the platform~$i$ is,
$$\MR_i(\VPhi; \beta) 
= \lambda_i(\VPhi; \beta) f(\phi_{i})\phi_{i} \left( 1 - \DA_i(\VPhi; \beta) \right) .$$
As $\lambda_i,$ and $\DA_i$ is jointly continuous, $\MR_i$ is also jointly continuous. \eop

\ignore{Now, as the objective function given in~\eqref{eqn_existence_uniq_WE_main} is jointly continuous over the compact domain, the existence of WE is guaranteed. Further, we define the WE and matching revenue (MR) of the limit system uniquely such that we have continuity as $\beta \to 0$. 
    %\item Next, we show the uniqueness of WE for the limit system, and
%(ii) next we show the continuity of WE.
%{\color{red} Even if there are multiple WE for limit system we need that the limit of $\PB(\beta)$ coincide with what we have used in the analysis.}
%W.l.o.g. let $\phi_1 > \phi_2$ which implies $f(\phi_1) < f(\phi_2)$. 
The procedure is as follows. We first find the minimizers of the objective function in~\eqref{eqn_existence_uniq_WE_main} using~$\PB(\VPhi;0)$ (given in~\eqref{Eq_overall_aproxx}) as limit QoS. 
Say at a particular~$\VPhi$,  these minimizers are unique. 
Then  continuity w.r.t.~$\beta$ follows from Maximum theorem~\cite{maximum}, as in the proof of Theorem~\ref{thm_monopoly_opt}, with additional advantage due to the unique optimizers: the upper semi-continuity of the correspondences of optimizers implies  continuity when they are further unique~(~\cite{maximum}). If the minimizers of limit system are  not unique, we pick an appropriate one from among, so as to ensure continuity (such a choice is again possible, because by Lemma~\ref{lem_exist_unique_WE}, WE are unique for~$\beta > 0$ and hence~$\lim_{\beta \to 0} W(\beta)$ {\color{red} define W} always exists). We call optimizers of~$W(0)$ as limit WE.
%then we choose the right minimizer such that the continuity is ensured. 
Once limit WE is found, we obtain limit MR using Lemma~\ref{lem_approx_MR}, and show it equals the ones provided in Table~\ref{tab:WE_MR_PB}. 
We proceed with the proof in the following steps.  

\textbf{Case 1: When $\phi_1 = \phi_2$:} From Lemma~\ref{lem_exist_unique_WE} and \eqref{Eq_overall_exact}, it is easy to see that the unique WE for $\beta > 0$ system is $(\lamo, \lamt) = (\Lambda/2, \Lambda/2).$ From \eqref{Eq_overall_aproxx}, for $(\lamol, \lamtl) = (\Lambda/2, \Lambda/2),$ we have $\PB_1(\VPhi;0) = \PB_2(\VPhi;0).$ Thus using Maximum theorem, $ W(\beta) \to W(0) = \Lambda/2.$

\ignore{We prove the uniqueness by contradiction. If possible, w.l.o.g., say there exists another limit WE with $\epsilon > 0$, such that
$$
(\lambda'_1(\VPhi),\lambda'_2(\VPhi)) = \left( \frac{\Lambda}{2}-\epsilon,\frac{\Lambda}{2}+\epsilon \right).
 $$
      One can easily verify from \eqref{Eq_overall_aproxx} that the blocking probabilities of the platform $1$ and $2$ are $\min\{1- \nicefrac{e}{\lambda'_1(\VPhi)}, 1-f(\phi_1)\}$ and $1-\nicefrac{e}{\lambda'_2(\VPhi)}$ respectively which can never be equal  since, $$\frac{e}{\lambda'_2(\VPhi)}<f(\phi_2)=f(\phi_1).$$
So, we have  unique minimizer of \eqref{eqn_existence_uniq_WE_main} for   limit system and for such $\VPhi$ (when $\PBl$ are equal, the optimal value  of  \eqref{eqn_existence_uniq_WE_main} is $ 0$).}
Substituting this WE in Lemma \ref{lem_approx_MR}, the matching revenue of the limit system equals,
 $$
    \MR_i(\VPhi; 0) = e\phi_i\mathds{1}_{\phi_i \in [0,f^{-1}\left( 2\rho \right))} + \frac{\Lambda}{2} f(\phi_i)\phi_i \mathds{1}_{\phi_i \in [f^{-1}\left( 2\rho \right),\phi_h]}.
$$
 % One can similarly argue for the WE with first platform obtaining $\epsilon$ higher arrival rate.

\textbf{Case 2: When $\phi_1 >  \phi_2$:}
\begin{enumerate}[$(a)$]
    \item  When $\phi_1, \phi_2 \in [0, f^{-1}\left( 2\rho \right))$: From the definition of $f^{-1}\left( 2\rho \right)$, we have $\nicefrac{2e}{\Lambda f(\phi_i)} < 1$ for any $i \in \{1,2\}$. Then, from~\eqref{Eq_overall_aproxx}, it is easy to see that the limit WE again equals, 
$\lamol = \Lambda/2$. To prove the uniqueness, say there exists another WE with $\epsilon>0$, such that
$$
(\lambda'_1(\VPhi; 0),\lambda'_2(\VPhi; 0)) = \left( \frac{\Lambda}{2}-\epsilon,\frac{\Lambda}{2}+\epsilon \right).
 $$
 %From \eqref{Eq_overall_aproxx}, the blocking probabilities of the platform $1$ and $2$ can be either $1-f(\phi_i)$ or $1-\nicefrac{e}{\lambda'_i(\VPhi)}$. Consider the following sub-cases:

\begin{itemize}
    \item When $\PB_1'(\VPhi; 0) = 1-f(\phi_1)$ and $\PB_2'(\VPhi; 0) = 1 -f(\phi_2)$:
 The above blocking probabilities can never be equal  since $f(\phi_1)\neq f(\phi_2)$.
 \item When $\PB_1'(\VPhi; 0) = 1-\nicefrac{e}{\lambda'_1(\VPhi; 0)}$ and $\PB_2'(\VPhi; 0) = 1-\nicefrac{e}{\lambda'_2(\VPhi; 0)}$: These cannot be equal since $\lambda'_1(\VPhi; 0)\neq \lambda'_2(\VPhi; 0)$.
 \item When $\PB_1'(\VPhi; 0) = 1 - f(\phi_1)$ and $\PB_2'(\VPhi; 0) = 1 -\nicefrac{e}{\lambda'_2(\VPhi; 0)}$: This case is also not possible since,
$$\frac{e}{\lambda'_2(\VPhi; 0)}<\frac{e}{\lamtl}=\frac{e}{\lamol} < f(\phi_1).$$
\end{itemize}
Similar logic follows for the remaining sub-case, and by Maximum theorem, $ W(\beta) \to W(0) = \Lambda/2$ (the unique limit WE, as given in Table \ref{tab:WE_MR_PB}).
%(iv) When $\PBl_1'=1-\nicefrac{e}{\lambda'_1(\VPhi)}$ and $\PBl_2'=1-f(\phi_2)$:
%This case is also not possible since,
%$$\frac{e}{\lambda'_1(\VPhi)}>\frac{e}{\lamo}=\frac{e}{\lamt}>f(\phi_2).$$
%
 %The unique limit WE for this case as given in Table \ref{tab:WE_MR_PB}.
%Using \eqref{eq_approx_MR} of 
Substituting this WE in Lemma \ref{lem_approx_MR}, the matching revenue of the limit system is, 
$
    (\MR_1(\VPhi; 0),\MR_2(\VPhi; 0)) = (e\phi_1, e\phi_2).
$

%{\color{red}Define $\phibar = f^{-1}\left(\frac{e}{\Lambda}\right)$.}

\item  When $\phi_1 \in [f^{-1}\left( 2\rho \right), f^{-1}\left( \rho \right))$, the limit WE   is given by,
\begin{equation} \label{eq_WE_b}
    \lamol   =  \left(\Lambda  - \nicefrac{e}{f(\phi_1)}\right).
\end{equation} 
 One can verify the above by directly substituting   in \eqref{Eq_overall_aproxx}; the resulting $\PB_1(\VPhi; 0),$ and $\PB_2(\VPhi; 0)$ are again equal and are given by $1- f(\phi_1)$ and $1 - \frac{e}{\lamtl}$ respectively. 

%the above claim by substituting the values in \eqref{Eq_overall_aproxx} and equating the blocking probabilities (see \eqref{eqn_existence_uniq_WE_main}) of the two platforms,
%In this case, note (see \eqref{}) that the blocking probabilities for platform 1 and platform 2 are 
%which turns out to be $1- f(\phi_1)$ and $1 - \frac{e}{\lamt}$ respectively. %{\footnote{This claim follows from the fact that the WE of the limit system is unique, which we prove later in this result.}}.
Next, we show that the above WE is the unique one. Towards this we first study $\PB_1(\lambda_1; 0)$ and $\PB_2 (\Lambda-\lambda_1; 0)$ of \eqref{Eq_overall_aproxx} as a function of $\lambda_1$.  With $x_1:=\nicefrac{e}{  f(\phi_1)}$ and 
$x_2:=\Lambda- \nicefrac{e}{  f(\phi_2)},$ 
\begin{align*}
    \PB_1(\lambda_1; 0) &= 1- \left(f(\phi_1) \mathds{1}_{ \lambda_1 \le x_1}  + \frac{e}{\lambda_1}   \mathds{1}_{ \lambda_1 > x_1}\right)  \\
     \PB_2(\lambda_1; 0) &=1- \left(f(\phi_2) \mathds{1}_{ \lambda_1 \ge x_2}  + \frac{e}{(\Lambda-\lambda_1)}   \mathds{1}_{ \lambda_1 < x_2}\right).
\end{align*}
Thus from~\eqref{eq_WE_b}, and $\phi_1 \geq f^{-1}\left( 2\rho \right)$; $\lamol \le x_1,$ and $\lamol < x_2$.  
And thus there can be no other $\lambda_1$ at which the two $\PB_i$ become equal: from the above equation, for all $\lambda_1 > \lamol$, $\PB_1 (\lambda_1; 0) > \PB_2 (\lambda_1; 0) $; the vice versa is true for $\lambda < \lamol$.  

Substituting this WE in Lemma \ref{lem_approx_MR}, the matching revenue of the limit system is,
$$
(\MR_1(\VPhi; 0),\MR_2(\VPhi; 0)) = ((\Lambda f(\phi_1)-e)\phi_1, e\phi_2).
$$
Observe $\lamol f(\phi_1)< e$ because $\phi_1 \ge f^{-1}\left( 2\rho \right)$ and so $f(\phi_1) \le 2e /\Lambda$.

\item  When $\phi_1 \in [f^{-1}\left( \rho \right), \phi_h]$, from \eqref{Eq_overall_aproxx} , $ \PB_1(\VPhi; 0) = 1 - f(\phi_1)$ irrespective of $\lamol$ while $\PB_2(\VPhi; 0) = \min\left\{ 1 - \frac{e}{\lamtl}, 1-f(\phi_2) \right \}$ where $\lamtl$ has to be found. Observe that for any $\lamtl$
$$
1-f(\phi_1) >1-f(\phi_2)\ge \min \left\{1 - \frac{e}{\lamtl}, 1 - f(\phi_2) \right\},
 $$
since $f(\phi_1) < f(\phi_2)$, and hence it is not possible to equate the blocking probabilities of the two platforms. 
In this case any $\lambda_1 $ optimizes \eqref{eqn_existence_uniq_WE_main}. 
Thus, we consider the following as limit WE:  
$$(\lamol, \lamtl) = \left(0, \Lambda \right),$$
and show that the selection ensures the required continuity properties. Towards this, consider any $\beta_n \to 0$ and consider corresponding $\lim_{\beta_n \to 0} W(\beta_n)$. We claim that $W(\beta_n) \to 0$, which we prove case-wise as below:
%i.e., the platform with the minimum blocking probability obtains the entire arriving streams of passengers. 
%To show the uniqueness of WE in this case, one needs to show that the WE $(\lamo,\lamt)$ corresponding to the sequence of $\beta_n \to 0$  converges to $(0,\Lambda)$, when $\phi_1 \in [\phibar, \phi_h]$ and $\phi_1>\phi_2$.
  
When $\phi_2 \in [f^{-1}\left( \rho \right), \phi_h]$:
Consider any $\epsilon >0.$
By   Lemma \ref{lem_approx_MR}, with $\lambda_i(\beta) = 0$
for all $\beta$,     
  there exists a $\beta_\epsilon$ such that 
  $$\DA_1 (\phi_1; 0, \beta) \le \epsilon/f(\phi_1)  \mbox{ and hence }
  \PB_1(\phi_1; 0,\beta) < 1-f(\phi_1) + \epsilon$$
  for all  $\beta \le \beta_\epsilon$ (see   \eqref{Eq_overall_exact}). In similar lines,  
  $$\PB_2(\phi_2; \Lambda,\beta) > 1-f(\phi_2)-\epsilon, \mbox{ when } \beta \le \beta_\epsilon.$$  This implies $\PB_1(\lambda;\beta) < 1-f(\phi_1) + \epsilon$ and $\PB_2(\lambda;\beta) \ge 1-f(\phi_2)-\epsilon$ respectively, for all $\lambda$. 
  %
For all such $0 < \beta \le \beta_\epsilon$ from \eqref{eqn_existence_uniq_WE_main},
$W(\beta)  = (0, \Lambda)$, if $\epsilon < (f(\phi_2) - f(\phi_1))/4$.

One can give similar arguments for the other case, now with $\PB_2(\phi_2;\Lambda,\beta) \to 1-\nicefrac{e}{\Lambda f(\phi_2)}$.
%\textbf{Case 2: When $f(\phi_2) > \nicefrac{e}{\lambda}$:}
This completes the proof of claim. 
Substituting this WE in Lemma \ref{lem_approx_MR}, the matching revenue is,
$$
(\MR_1(\VPhi; 0),\MR_2(\VPhi; 0)) = (0,\min \{\Lambda f(\phi_2),e\} \phi_2). 
$$
\end{enumerate}
\eop
}
}

